Dynamic Prompt Middleware: Contextual Prompt Refinement Controls for Comprehension Tasks

Effective prompting of generative AI is challenging for many users, particularly in expressing context for comprehension tasks such as explaining spreadsheet formulas, Python code, and text passages. Prompt middleware aims to address this barrier by assisting in prompt construction, but barriers remain for users in expressing adequate control so that they can receive AI-responses that match their preferences. We conduct a formative survey (n=38) investigating user needs for control over AI-generated explanations in comprehension tasks, which uncovers a trade-off between standardized but predictable support for prompting, and adaptive but unpredictable support tailored to the user and task. To explore this trade-off, we implement two prompt middleware approaches: Dynamic Prompt Refinement Control (Dynamic PRC) and Static Prompt Refinement Control (Static PRC). The Dynamic PRC approach generates context-specific UI elements that provide prompt refinements based on the user's prompt and user needs from the AI, while the Static PRC approach offers a preset list of generally applicable refinements. We evaluate these two approaches with a controlled user study (n=16) to assess the impact of these approaches on user control of AI responses for crafting better explanations. Results show a preference for the Dynamic PRC approach as it afforded more control, lowered barriers to providing context, and encouraged exploration and reflection of the tasks, but that reasoning about the effects of different generated controls on the final output remains challenging. Drawing on participant feedback, we discuss design implications for future Dynamic PRC systems that enhance user control of AI responses. Our findings suggest that dynamic prompt middleware can improve the user experience of generative AI workflows by affording greater control and guide users to a better AI response.

==> tables/ImproveDesign.tex <==
0                                                                                                     Could you save the particular set of preferences like a personal bookmark?
1                                                                                                     Reading the description of preferences and their different output in parallel helps greatly to understand the different preferences.
2                                                                                                     One would be to allow users to save a preference and not need to do this every time, while allowing users to change that if the context changes.
3                                                                                                     Perhaps formatting, use of color for example.
4                                                                                                     "Other" field for each selection. "Output type" that the output is generated by Microsoft PowerPoint slide.
5                                                                                                     Make it conversational instead of combos and radios. The manual input should be the fallback
6                                                                                                     the length of the prompt. everything is amazing :) 
7                                                                                                     overview for the steps taken
8                                                                                                     Cannot think of anything
9                                                                                                     The description of "Role of AI explanations" is unclear. It feels like this correlates with Novice/Intermediate/Expert but I'm not sure if it does? \nI'm not sure what length or time refers to. Is is the time the AI takes to generate an explanation? The character length of the explanation?
10                                                                                                                    
11                                                                                                    Nothing
12                                                                                                    The characteristics of AI explanations that I would want could evolve while doing the same task. It would be nice if I don't have to actively push buttons for this and just dynamically and naturally change as I speak with the AI assistant.
13                                                                                                    option for visuals - charts
14                                                                                                    I think Design C fulfill my expectations
15                                                                                                    Rather than default settings that are controlled by the user. An AI that remembers topics i usually struggle on and prompt for more information or topics i don't usually struggle on and changes the content automatically. Or to accept prompts like, teach me quickly, tell me in short, give me 80% of the teachings in 20% of content. 
16                                                                                                    i can't think of such. it looks good
17                                                                                                    not sure I understand this question
18                                                                                                    remember my selection 
19                                                                                                    Fewer choices. Perhaps light, medium, detailed.
20                                                                                                    Sourcing control (LLM-only, Current document, company sharepoint resources, public web resources.
21                                                                                                    Maybe let users select prior to uploading the data set, and then users can adjust their selections after seeing the AI results. 
22                                                                                                    I like the design -- I would just like it to be an option to go into that selection process (like the function wizard).
23                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     no idea
24                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         nan
25                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         maybe a smoother UI
26                                                                                                    I think there should be like 3 settings, basic - intermediate - expert and you could just set which level you're at. The setting would dictate whether you got text or images and most or all should offer up the video link if available.
27                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         Yes
28                                                                                                    Add ability to request for key insights from the end result (or data analaysis), could be a choice of 1 or 3 or 5 insigts for example
29                                                                                                                                                                                                                                                                                                                                                                                                                                           being able to control temperature, data sets (e.g. time created and age of documentation used).\n
30                                                                                                    That I am able to set my default preferences with the option to change everything in a dialog with AI at any time  
31                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                Nothing else comes to mind. 
32                                                                                                                                                                                                                                                                                                                         In a way. But I wouldn't want to spend time in the beginning to adjust the level of explanations. When I jump into a task, I just want to get it done as soon as possible, so I don't want any additional hurdles. 
33                                                                                                                                                                                                                                                                                                                      I strongly dislike the natural language prompt to select preferences. It's a waste of time to type in my goal for the AI to get my preferences wrong when I could just click a bunch of radio buttons and check boxes.
34                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        I prefer the "Explain to me" option.
35    Related to the above - some settings may just be more general and would not have to be asked for each interaction.\n\nOne thing that I would particularly like to have control over is to be able to easily direct the AI's explanation towards aspects that do not seem right to me or that just seem worth taking a closer look at (e.g. the surprisingly pronounced spike in shark attacks in 1905). In other words, the AI might not always need to explain the whole analysis to me but just specific steps or parts of the output.
36                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               Maybe a video
37                                                                                                                                            Instead of categories, potentially showing a slider that gives me more finegrained control. However I'm unsure if that would add too much cognitive load, and if more control is necessarily better. Another way would be for me to interact with the model through a CUI and point to existing text blogs and ask it to explain to me in the style of that blog. Again, might be too much work.
Name: What would enhance Design C to better assist in your CONTROL of AI explanations?, dtype: object

==> tables/OtherFeatures.tex <==
0                                                                                                     Could the AI assess the prompt quality? For instance some sort of RAG system.
1                                                                                                     point out data anomalies ? in the task examples it is clear what the source of the data is. I can imagine a lot of examples where this is far more complicated. 
2                                                                                                     An interface where when the AI makes assumptions (e.g. "Assumption 1: US locations will be 'Atlantic Ocean'", the user can see each one and have the ability to accept or reject/alter them. 
3                                                                                                     I like the idea of starting out simple and being able to go deeper into AI explanations.
4                                                                                                     To keep the output for next time, that is the storage function that user can go back to the previous output from AI assistant.
5                                                                                                     
6                                                                                                     i love the recommendation to continue the talk and interpreting the data 
7                                                                                                     videos from similar cases
8                                                                                                     nan
9                                                                                                     Call out when the info comes directly from my dataset, vs being augmented by other datasets / web searches
10                                                                                                                                              
11                                                                                                    Nothing
12                                                                                                    Interactive plots, seamless integration between apps (imagine if I can click on the plot and get redirected to the apps where I could interactively change things)
13                                                                                                    na
14                                                                                                    None
15                                                                                                    None that i haven't already mentioned. 
16                                                                                                    i can't think of such.
17                                                                                                    Im pretty happy with how it is progressing, I don't think about it enough to have an opinion, I just use it :)
18                                                                                                    shorts 15 sec videos 
19                                                                                                    Having less of the explanation in-line and cluttering the UX ... and instead offer via off-site links.
20                                                                                                    When I ask the AI to elaborate, sometimes an AI will just repeat it self. Even when I point out the AI is repeating itself it will continue. That's not really useful is it? An improvement would be for the AI to find another way of explaining.
21                                                                                                    Maybe a prompt by AI to ensure concepts are clear; maybe a little task from AI so I can try out my new knowledge. 
22                                                                                                    Perhaps linking to "help" content as well. I still use "help" resources including application documentation and forums. That would also prompt people to connect with peers as they experiment and validate AI tools.
23                                                                                                    examples are enough
24                                                                                                    nan
25                                                                                                    something that links to source documents. 
26                                                                                                    I didn't know there were even explanations available so maybe letting users know when they start using the AI that they can "click here" for explanations would be helpful.
27                                                                                                    it seems Design C also helps with prompting for AI which can affect the AI results.  
28                                                                                                    Ability to let the AI refine to use multiple column data for analysis, plotting etc. as most often just one attribute is not enough
29                                                                                                     being able to actually know the data set being used.  Possibly being able add additional data sets.  if the findings are inferred, then noting that and how and why it inferred it. 
30                                                                                                    AI should be able to learn my preferences without a UI. Seems old-school to use GUI where NLUI makes more sense 
31                                                                                                    As above, I think it might be useful sometimes to have a notebook-like output which combines (1) steps that AI took, (2) outputs it produced at each step, (3) explanations for each step. This might be helpful to review for complex workflows, as the chat interface is small/narrow and harder to navigate. 
32                                                                                                    If it could learn my level of statistical knowledge overtime. Essentially personalize the experience to me. 
33                                                                                                    The option to have a step-by-step walkthrough of how I can achieve the same result using the application interface. Not a tutorial, but a guide (go to this menu, click on this button, write this formula, etc.)
34                                                                                                    More options of the shown designs - for example adding more charts options that can explain the data...
35                                                                                                    Linking what it does directly to the GUI. For example, when it does a suggested analysis, you could ask the AI to actually do it within the GUI of Excel as if it were a tutorial.
36                                                                                                    I don't know
37    
I would love to see visualizations of decisions, including alternative paths that the process could have taken. If we made a different decision along the way (e.g. analysis A vs. analysis B), how does that change the output and how it is reported? Does one vs. the other fit better with the narrative I'm building? This question is more for me since I have that knowledge (i.e. what I'm trying to do with the output of the data outside  of Excel).
Name: What other features or improvements to AI explanations might assist you in understanding AI assistance?, dtype: object

==> tables/WhatToControl.tex <==
0                                                                                                     The ones shown would work well.
1                                                                                                     subtle difference between characteristics of "coach me", "teach me", "explain to me" - is not easy to understand for non-natives - so doesn't matter. Length or type of explanation is important. the others - depends if it is more difficult task, i presume.
2                                                                                                     Video is king, and choosing level of expertise (e.g. "I don't know how to code") would be most important.
3                                                                                                     naming/text first and images second.
4                                                                                                     Everything listed in the CONTROL. For a role of AI explanation, I would want more choices like "as a data scientist". 
5                                                                                                     type and complexity
6                                                                                                     explain to me was the best because i save time and i get to know the final results. If I will use AI often then I don't need to know all the process behind 
7                                                                                                                                                                                                                                                                                                                                                                         type of explanation and level of details, and steps taken
8                                                                                                                                                                                                                                                                                                                                                                                                                               all
9                                                                                                                                                                                                                                                                                                                     Level of expertise, type of explanation (I am hard-of-hearing so videos don't work unless they are captioned)
10                                                                                                                                                                                                                                                                                                                                                                                                                                 
11                                                                                                                                                                                                                                                                                                                                                                                                                              All
12                                                                                                                                                                                                                                                                                                                                                                        yes, type of explanation, level, length are all important
13                                                                                                                                                                                                                                                                                                                                                                                          the length, tone, visual representation
14                                                                                                                                                                                                                                                                                                                                                                                                                  Text and images
15                                                                                                                                                                                                                                                                                                                                                                                                   The ones listed in the example
16                                                                                                                                                                                                                                                                                                                                                                                                              all those mentioned
17                                                                                                                                                                                                                                                                                                                                                                                  Chatty style, not too robotic, short and punchy
18                                                                                                                                                                                                                                                                                                                                                                                                                             all 
19                                                                                                                                                                                                                                                                                                                                                                                        Length of explanation and expertise level
20    formality, length, type of response, attention to detail, and most importantly: whether or not the model should utilize external sources when building a response!! Sometimes I only want the model to generate a response internally, in the LLM itself, using the 'knowledge' that exists in the neural net. There's not always the need to go looking at the document, go looking on the web, or go looking in sharepoint.
21                                                                                                                                                                                                                                                                                                                                                                   All of them seemed important to create a tailored experience. 
22                                                                                                                                                                                                                                                                                         I'm not sure. It would be a trade off -- I'm willing to give up some control to not have to go through too many choices in getting ther.
23                                                                                                                                                                                                                                                                                                                                                                                                                  text and images
24                                                                                                                                                                                                                                                                                                                                             level of expertise first, then length of explanation, and then type of explanation/ 
25                                                                                                                                                                                                                                                                                                                                                                                    length of explanation and type of explanation
26                                                                                                                                                                                                                                                                                I think it's a bit too much. I think there should be like 3 settings, basic - intermediate - expert and you could just set which level you're at.
27                                                                                                                                                                                                                                                                                                                                                                                       type of explanation and level of expertise
28                                                                                                                                                                                                                                                                         All of these are important, love the idea of recommendation... but should have the ability to update any of these attributes to manage my own experience
29                                                                                                                                                                                                                                                                                                                                quick should have short where as a detailed description should have a longer in depth tutorial.  
30                                                                                                                                                                                                                                                                                     that I control what I want AND that it is flexible. Depending on the task, I may have different preferences and it must be simple to change 
31                                                                                                                 All of those listed in the question, and also:\n- "conciseness of language used" (related to length, but this is more about using full sentences etc. vs. just giving me the bare facts). \n- interactivity (e.g., whether each explanation is dynamically linked to some element of the spreadsheet interface) 
32                                                                                                                                                                                                                                                                                 The specific formula it has deployed, and why it's the appropriate formula/statistical approach to solving the specific problem I'm working on. 
33                                                                                                                                                                                                                                                                                                                                         Level of expertise, role, format. Not length or time, which is hard to judge in advance.
34                                                                                                                                                                                                                                                                                                                                                                                    Images & videos- preferred short descriptions
35                                                                                                                                  All the choices make sense. However, some of the settings may be general preferences that could be set somewhere in the AI assistant's settings (e.g. "Include media types" or "Start with" options) and some may be more activity-specific and set for each task/spreadsheet someone works on.
36                                                                                                                                                                                                                                                                                                                                                                                                    Short text, images and videos
37                                                                                                                                                                                                                                                                                                                                                             Length, expertise, and explanation type (end result vs. modular etc)
Name: What characteristics of AI explanations is it important for you to have control over?, dtype: object

==> tables/WhyControlResponses.tex <==
0  (+1 to all for PNUMS)
I think the settings approach seems like a good way forward however, I would need to try it to see if it becomes an unwanted overhead. 
1                                                                                              
having control allows you to understand the data analysis to a level where you can explain to others (if required)
2 
This adapts to the user in the context of their daily work. Maybe they're trying to learn how to use pivot tables, in this case they'd choose "Coach Me". In other cases, they're running a routine monthly report and need the most basic explanations. Every time a user sits down with Excel, the context, pressure, complexity and novelty will change.
3                                                                                              
C provided the type of visual and level of control I would like to have.
4                                                                                              
Ultimately the goal of the task is not the same. The output can be better fit to the prompt if user can CONTROL how the AI assistant work.
5                                                                                              
Not sure
6                                                                                              
I could add a prompt and there was option how I want the data to be analyze 
7                                                                                              
for some of the tasks more details are needed, on these cases it would be great to have the option to change the control. to have more details for tasks that are difficult for me to understand
8                                                                                      
I do like this Design feature but would want to be in control of when it was available to assist with the AI prompt.  I think if I had to use this everytime I would get frustrated.  I am guessing that using this type of prompt would enable the AI to learn more about my aptitude of the platform
9                                                                                              
be nice, but I'd prefer the defaults to be good. If the AI is treating me like a novice while I'm an expert, I'd expect to be able to tell the AI to stop via the chat interface, not settings.
10
(nothing)
11                                                                                             
Because I have tasks with a range of expertise, so I'll want to control the AI's teaching to different tasks.
12                                                                                             (answered in previous question)
13                                                                                             
expectation of getting better responses. 
14                                                                                             
It gives more options for the user to tailor their expected outcomes
15                                                                                            
This gives me some default control to customize the responses i will receive and may fit better with my learning style.  
16                                                                                             In some tasks I would like to understand how it was calculated and on some I wouldn't 
17                                                                                             
wishywashy response, but I'm not sure I'm that bothered.  Depends on which AI it is Im using whether I full trust it.  If its Copilot, I trust that, some others I would not so much and would want more control
18                                                                                             
for experts you need to have flexibility 
19    
This model feels overly heavy, too many choices, and geeky. It feels like something Microsoft made as opposed to something Apple made. Feels like poor usability. I don't want to go through a whole menu of choices and options and explanations of the radio buttons ... I just want Microsoft smart designers to make the best thing and put it forward. Then learn via A/B testing.
20                                                                                             
I want the AI to respond in a predictable manner. I don't want to repeat myself each time, or do minor adjustments to the prompt manually.
21                                                                                             
It lets you tailor the experience to your specific needs. 
22                                                                                             
I think this would be helpful if it were optional to turn it on -- like using the function wizard in Excel. I don't need it all the time, but it sure is helpful when I do need it.
23                                                                                             
It is good if you have several options you can choose from depending on the use case you work at ---just information for a team meeting or exec meeting for example
24                                                                                             
Understanding the steps allows for validation and builds trust in the AI. Being able to adjust the level of detail based on the concepts I'm familiar with would be an excellent feature! 
25                                                                                             
this would be good, but not if i have to set it every time
26                                                                                            
At first I was a bit put off by the number of settings. But I do think the degree of control on the explanation is important. 
27                                                                                            
Like the options and puts me in control
28                                                                                             
Flexible options based on the task involved and our experience/understanding of those concepts is critical.
29                                                                                            
If its a new concept or area that I am not familiar with, I would like more detailed info.  If looking for a quick answer I'm too lazy to work out, then a quick answer is what I'm looking for. 
30                                                                                             
aligned with my previous responses
31                                                                                             
Different levels of explanation are relevant for different contexts, so I want to be able to control this. 
32                                                                                             
The AI has no context on how much or little I know about spreadsheets, so it shouldn't make any assumptions. 
33                                                                                             
I want control but I don't want this to be in the way. I.e. when I work in a new document, I don't want to have a pop-up asking me what kind of explanations I want.
34                                                                                             
I see there is a different propose for each level of detail.
35                                                                                             
The needs for explanation will differ depending on the task, goals, and the available time frame so having control makes sense.
36                                                                                             I'm not sure I fully understood this scenario to have a strong opinion about it 
37                                                                                             Changing the role of AI explanation seems like a good start in customizing for my own needs. Could go a step further (with my own custom input to the model for what I want), but that might be a lot of work for me.
Name: Why did you choose the answer to the above question?5, dtype: object

==> text/ExplanationDetailLevelJSON.tex <==
[
  {
    type: "option",
    label: "Explanation Detail Level",
    description: "Choose the level of detail for the explanation",
    options: {
      Basic: "Provide a basic explanation of the formula components",
      Intermediate: "Include a more detailed explanation with examples",
      Advanced: "Offer an in-depth explanation with potential use cases",
    },
    appearance: "single-select-radio",
    value: "Provide a basic explanation of the formula components",
    reason: "Allows the user to select the depth of explanation they need for understanding the formula.",
  },
]
